Dynamic Wetting by Concentrated Granular Suspensions

Many functional materials, such as paints and inks used in applications like coating and 3D printing, are concentrated granular suspensions. In such systems, the contact line dynamics and the internal structure of the suspension interact through shear rate dependent viscosity and microstructural rearrangements. The local shear rate increases sharply near moving contact lines, leading to the non-Newtonian rheology of dense suspensions in this region. While hydrodynamic solutions can describe dilute suspensions, their applicability near advancing contact lines in dense suspensions remains unclear. This study quantifies the deviation from the Newtonian solution by systematically varying interparticle interactions through the choice of dispersion medium. We use silica particles suspended in two refractive index-matched fluids: (i) aqueous 2,2'-thiodiethanol (weak interactions) and (ii) aqueous sodium thiocyanate solution (strong interactions). These systems exhibit substantially different rheological responses, shear-thickening and yield-stress behaviour, respectively. Using astigmatism particle tracking velocimetry (APTV), we resolve the three-dimensional trajectories of tracer particles within a drop driven over a substrate, in an arrangement enabling tracking the internal flows over a long travel distance of the drop. We observe distinct flow behaviours depending on the particle interactions and the resulting suspension rheology. The more the particle interactions play a role, i.e., the more pronounced the non-Newtonian effects are, the stronger the measured flow profiles differ from the Newtonian solution to the hydrodynamic equations. In the shear-thickening suspension, a notable deviation from Newtonian behaviour is observed. Conversely, the yield-stress suspension exhibits plug flow over the substrate, with Newtonian-like behaviour restricted to the yielded region near the substrate.

==> latexmkrc <==
$sub_doc_output = 'output-subdoc';

@sub_doc_options = ();

push @sub_doc_options, '-pdf'; # Use pdflatex for compilation of external documents.
# Replace '-pdf' by '-pdfdvi', 'pdfxe', or 'pdflua' if needed.

push @file_not_found, '^No file\\s*(.+)\s*$';

add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );
sub makeexternaldocument {
    if ( $root_filename ne $_[0] )  {
        my ($base_name, $path) = fileparse( $_[0] );
        pushd $path;
        my $return = system "latexmk",
                            @sub_doc_options,
                            "-aux-directory=$sub_doc_output",
                            "-output-directory=$sub_doc_output",
                            $base_name;
        if ( ($sub_doc_output ne ' ') && ($sub_doc_output ne '.') ) {

             rdb_add_generated( "$sub_doc_output/$base_name.aux" );
             copy "$sub_doc_output/$base_name.aux", ".";
        }
        popd;
        return $return;
   }
}
